AIRGuard: Guarding Agent Actions with Runtime Authority Control

Tool-using language agents turn model decisions into external side effects: they read files, run scripts, call APIs, send messages, and invoke Model Context Protocol tools. This makes agent attacks different from jailbreaks. The harmful step is often not an obviously forbidden output, but an ordinary executable action that becomes unsafe because attacker-controlled context steers authorized access against the user's interest. We identify this failure mode as authority confusion: untrusted resources may inform reasoning, but they must not authorize side effects. We present AIRGuard, a runtime guard that operationalizes least privilege as action-time authorization. AIRGuard normalizes heterogeneous tool calls, derives task authority into step-level authority, tracks source and target trust, simulates sensitive side effects, audits cross-step risk, and enforces decisions before actions execute. On AgentTrap, AIRGuard reduces Sonnet 4.6 attack success from 36.3% without defense to 5.5%. On DTAP-150, AIRGuard preserves 76.0% benign utility with Haiku 4.5, compared with 52.0% for ARGUS and 42.0% for MELON. An ablation further shows that prompt-only policy helps only modestly, whereas a dedicated runtime authority-control layer gives the agent system direct control over tool-mediated side effects. Code and data are available at https://github.com/Sophie508/AIRGuard.

==> figures/fig_motivation.tex <==
\begin{figure*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tikzpicture}[
    font=\small,
    node distance=0.9cm and 1.0cm,
    box/.style={draw, rounded corners=2pt, align=center, inner sep=5pt, minimum height=1.0cm},
    trusted/.style={box, fill=green!8, draw=green!45!black, text width=2.8cm},
    untrusted/.style={box, fill=red!6, draw=red!55!black, text width=2.9cm},
    agent/.style={box, fill=blue!7, draw=blue!55!black, text width=2.6cm, minimum height=1.25cm},
    action/.style={box, fill=orange!9, draw=orange!70!black, text width=2.7cm},
    guard/.style={box, fill=gray!8, draw=black!55, text width=3.0cm, minimum height=1.25cm},
    ok/.style={-Latex, thick, draw=green!45!black},
    bad/.style={-Latex, thick, draw=red!65!black},
    flow/.style={-Latex, thick, draw=black!65}
]

\node[trusted] (authority) {Trusted authority\\user task / policy\\explicit consent};
\node[untrusted, below=of authority] (resource) {Untrusted resource\\webpage / file\\MCP output};
\node[agent, right=1.2cm of $(authority)!0.5!(resource)$] (agent) {Tool-using\\agent};
\node[action, right=1.1cm of agent] (proposal) {Proposed side effect\\tool call / command\\API action};
\node[guard, right=1.0cm of proposal] (guard) {\systemname{} check\\Does authority cover\\this target and effect?};
\node[trusted, right=1.0cm of guard, yshift=0.65cm] (allow) {Execute\\authorized action};
\node[untrusted, right=1.0cm of guard, yshift=-0.65cm] (block) {Block / inspect\\authority confusion};

\draw[ok] (authority.east) -- node[above, sloped, font=\footnotesize] {may authorize} (agent.west);
\draw[bad] (resource.east) -- node[below, sloped, font=\footnotesize] {may inform} (agent.west);
\draw[flow] (agent.east) -- (proposal.west);
\draw[flow] (proposal.east) -- (guard.west);
\draw[ok] (guard.east) -- (allow.west);
\draw[bad] (guard.east) -- (block.west);

\node[draw=red!55!black, dashed, rounded corners=2pt, fit=(resource) (agent) (proposal), inner sep=7pt,
      label={[font=\footnotesize, text=red!55!black]below:unsafe path: untrusted content becomes the reason for a side effect}] {};
\end{tikzpicture}
}
\caption{Motivation: authority confusion occurs when untrusted content is allowed to authorize side effects. \systemname{} preserves the distinction between information that may guide the agent and authority that can justify an action.}
\label{fig:motivation}
\end{figure*}


==> figures/fig_pipeline.tex <==
\begin{figure*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tikzpicture}[
    font=\small,
    node distance=0.55cm,
    stage/.style={draw, rounded corners=2pt, align=center, inner sep=5pt, minimum height=1.0cm, text width=2.25cm, fill=blue!6, draw=blue!55!black},
    decision/.style={draw, diamond, aspect=1.8, align=center, inner sep=2pt, text width=1.9cm, fill=orange!9, draw=orange!75!black},
    output/.style={draw, rounded corners=2pt, align=center, inner sep=5pt, minimum height=0.9cm, text width=2.0cm, fill=green!8, draw=green!45!black},
    block/.style={draw, rounded corners=2pt, align=center, inner sep=5pt, minimum height=0.9cm, text width=2.0cm, fill=red!6, draw=red!55!black},
    audit/.style={draw, rounded corners=2pt, align=center, inner sep=5pt, minimum height=0.9cm, text width=2.25cm, fill=gray!9, draw=black!55},
    arrow/.style={-Latex, thick, draw=black!65}
]

\node[stage] (intercept) {Intercept proposed action};
\node[stage, right=of intercept] (normalize) {Normalize action\\and target};
\node[stage, right=of normalize] (authority) {Extract authority\\context};
\node[stage, right=of authority] (trust) {Label resource\\and target trust};
\node[stage, right=of trust] (risk) {Simulate likely\\effect and tags};
\node[decision, right=0.75cm of risk] (enforce) {Policy\\enforcement};

\node[output, right=0.9cm of enforce, yshift=0.8cm] (allow) {Allow / audit};
\node[audit, right=0.9cm of enforce] (inspect) {Ask / inspect\\sandbox / quarantine};
\node[block, right=0.9cm of enforce, yshift=-0.8cm] (deny) {Block};
\node[audit, below=1.0cm of $(authority)!0.5!(risk)$] (ledger) {Action ledger\\sequence audit};

\draw[arrow] (intercept) -- (normalize);
\draw[arrow] (normalize) -- (authority);
\draw[arrow] (authority) -- (trust);
\draw[arrow] (trust) -- (risk);
\draw[arrow] (risk) -- (enforce);
\draw[arrow] (enforce) -- (allow.west);
\draw[arrow] (enforce) -- (inspect.west);
\draw[arrow] (enforce) -- (deny.west);

\draw[arrow] (normalize.south) |- (ledger.west);
\draw[arrow] (trust.south) -- (ledger.north);
\draw[arrow] (risk.south) |- (ledger.east);
\draw[arrow] (ledger.east) -| (enforce.south);

\node[draw=black!45, dashed, rounded corners=2pt, fit=(authority) (trust) (risk), inner sep=7pt,
      label={[font=\footnotesize, text=black!70]above:authority and risk are evaluated before execution}] {};
\node[font=\footnotesize, align=center, text=black!70, below=0.25cm of ledger]
      {Risk simulation can raise concern, but cannot grant missing authority.};
\end{tikzpicture}
}
\caption{\systemname{} pipeline. The guard converts heterogeneous tool calls into normalized actions, checks whether the current authority covers the target and likely effect, then applies tiered enforcement while recording evidence for sequence-level audit.}
\label{fig:pipeline}
\end{figure*}


==> sections/04_implementation.tex <==
\section{Implementation}

We implement \systemname{} as a Python runtime package with adapters for two agent substrates.
The core entry point, \texttt{check\_action}, runs the five-layer pipeline: resource labeling, target trust assessment, authority coverage, risk simulation, enforcement, and sequence audit.
The guard returns an outcome and a structured rationale, allowing wrappers to block, audit, or forward a tool call.
Every decision includes the normalized action, authority coverage result, risk tags, risk-simulation source, target trust tier, and enforcement outcome.
This makes failures inspectable: a blocked legal filing, for example, can be traced to a secrets tag, target-trust judgment, or missing capability rather than a generic model refusal.

\paragraph{AgentTrap integration.}
AgentTrap cases run in isolated Docker workspaces with tools such as file read, file write, script execution, shell commands, and final response.
\systemname{} maps these tools to normalized actions.
The native CLI integration records AIRGuard decisions into tool logs and filters blocked tool calls so that blocked attack-path calls do not count as executed side effects.

\paragraph{DTAP integration.}
DTAP exposes domain tasks through MCP servers.
\systemname{} wraps the upstream MCP server with a transparent proxy.
The proxy receives each tool call, normalizes the tool and arguments, checks authority and risk, blocks denied calls before execution, forwards allowed calls to the original MCP server, and redacts sensitive output when needed.
This lets the same guard mediate domains such as code, OS filesystem, finance, legal, and telecom without modifying each domain server.

\paragraph{Policy choices.}
The implementation uses conservative defaults.
Read and write are allowed for routine workspace tasks; exec and network require stronger authority or inspection.
Unknown MCP tools are treated as API calls rather than local code execution, avoiding a false-positive pattern where domain-specific read tools were blocked as exec.
High-risk tags include secrets, persistence, destructive write, hidden recipient, unauthorized network, privilege escalation, download-execute, and config poisoning.
For example, an \texttt{email.send} call with an unrequested BCC receives a hidden-recipient tag; if the recipient was introduced by low-trust content rather than user authority, the call is blocked before it reaches the mail tool.

\paragraph{Known implementation caveats.}
The current DTAP Claude CLI runs use the MCP proxy and deterministic policy, but the full LLM risk simulator is not always active.
Some low-level containment mechanisms, such as copy-on-write filesystems and rollback metadata, are represented in design and logs but not fully implemented.
Thus our evaluation should be read as a runtime-mediation prototype, not as a complete production security system.

